ETVO: Effectively Measuring Tactile Internet with Experimental Validation

The next frontier in communications is teleoperation -- manipulation and control of remote environments with feedback. Compared to conventional networked applications, teleoperation poses widely different requirements, ultra-low latency (ULL) is primary. Realizing ULL communication demands significant redesign of conventional networking techniques, and the network infrastructure envisioned for achieving this is termed as Tactile Internet (TI). The design of the network infrastructure and meaningful performance metrics are crucial for seamless TI communication. However, existing performance metrics fall severely short of comprehensively characterizing TI performance. We take the first step towards bridging this gap. We take Dynamic Time Warping(DTW) as the basis of our work and identify necessary changes for characterizing TI performance. Through substantial refinements to DTW, we design Effective Time- and Value-Offset (ETVO) -- a new method for measuring the fine-grained performance of TI systems. Through an in-depth objective analysis, we demonstrate the improvements of ETVO over DTW. Through human-in-the-loop subjective experiments, we demonstrate how and why existing QoS and QoE methods fall short of estimating the TI session performance accurately. Using subjective experiments, we demonstrate the behavior of the proposed metrics, their ability to match theoretically derived performance, and finally their ability to reflect user satisfaction in a practical setting. The results are highly encouraging.

==> sec/acknowledgements.tex <==
% \section{Acknowledgments}
This project is supported by SCOTT that has received funding from the Electronic Component Systems for European Leadership Joint Undertaking under grant agreement No 737422 http://www.scottproject.eu. This joint undertaking receives support from the European Unions Horizon 2020 research and innovation program and Austria, Spain, Finland, Ireland, Sweden, Germany, Poland, Portugal, Netherlands, Belgium, Norway.


==> sec/experimentalsetup.tex <==
\section{Experimental setup}\label{sec:setup}
To validate our proposed metric, we develop a realistic TI testbed, where a human user can interact with a remotely rendered virtual environment (VE) over a real network. We consider a recently proposed testbed for simulating TI interaction (Section~\ref{subsec:stdsetup}). This testbed lacks a network and is therefore not suited for mimicking TI interactions. Hence we carry out significant refinements to realize a networked TI testbed to provide a more comfortable TI experience (see Section~\ref{subsec:newsetup}).
%
\subsection{Standard TI testbed} \label{subsec:stdsetup}
% \input{5_experimentalsetup/fig_basesetup.tex}
The standard TI testbed proposed recently by Bhardwaj et al. simulates a TI session by having the human participant interact with a VE via both haptic and visual feedback \cite{Bhardwaj2017}. The haptic device is sampled at a rate of \SI{1}{kHz} and the VE is able to produce a \SI{1}{kHz} signal which is sent back as force feedback to the haptic device. A visual rendering of VE is also produced, but at the significantly slower rate of \SI{60}{Hz}. A schematic overview of this setup is indicated as the gray blocks in Figure~\ref{fig:setup}. The haptic device used in this setup is a Novint Falcon \cite{novintfalcon}. Force calculation and rendering in the VE is implemented inside of Chai3D \cite{Chai3dfeatures}, where force calculations are performed by the bullet real-time physics engine \cite{bulletengine}. In the application a virtual block with a specified mass can be pushed around over a virtual hard surface. It should be noted that this application does not support communication and runs everything in one program. Therefore, without improvements this testbed does not function as a valid testbed for TI. 
%
\subsection{Networked TI testbed}\label{subsec:newsetup}
We extend the aforementioned testbed by decoupling the testbed into an operator and a teleoperator, each residing on a different workstation, connected by a network. 
%
The operator measures the position of the ball the human is moving around and provides feedback to the human in the form of force feedback that is applied to the ball by the Novint Falcon, and visual feedback on the monitor based on data received from the feedback channel. The teleoperator houses the physics simulation. The physics simulation is a substitute for a TI application where the teleoperator would house a real physical environment with a physical robot arm. The teleoperator receives packets from the feedforward channel and feeds them into the physics environment. Then the location and orientation of all dynamic objects, as well as the calculated force are sent over the feedback channel to the operator. The operator receives the force feedback data and gives that to the Novint Falcon. Besides that, all the position and orientation values are used to displace all dynamic objects locally, and then an image is rendered. Because the video data is rendered at the operator, we overcome the need for live video transmission. This is a conscious decision, as it allows the research to focus on haptic feedback, and allows the challenge of low delay video transmission to be solved separately. An overview of the entire system is shown in Figure \ref{fig:setup}. 

\begin{figure}[t]
\centering
\includegraphics[width=0.499\textwidth]{fig/tikz.pdf}
\caption{A schematic overview of our experimental setup. The two dashed boxes indicate different applications that can run on different computers that are spatially distant. The Bullet physics engine operates in a different system than the operator, resembling a real TI system. The haptic device used is a Novint Falcon and the application is built on Chai3D. Instead of rendering an image in the remote environment, the position and rotation of all movable objects are transmitted. A local renderer in the operator system is used to generate the image locally. Because of this, the burden of bandwidth requirement of video transmission can be ignored in this setup. This way the system can isolate on the effects of kinesthetic and force information.}
\label{fig:setup}
\vspace{-8pt}
\end{figure}
For the user study performed Netem is used to simulate various network conditions, which ensures strong control over the network performance. This control is desirable, as the main purpose of the experiment is to analyze the performance of ETVO with respect to various network configurations.
%
During the experiment human operators are subjected to several instances of the same scenario that are subject to different network settings simulated with Netem. In order to perform an extensive performance evaluation of ETVO, we consider a wide variety of network conditions with respect to: constant delay, uniform packet loss, and bursty packet loss. In addition to considering these parameters in isolation, we also consider combinations of these parameters for realistic performance assessment of ETVO. The burst packet loss makes use of the Netem built-in Gilbert-Elliot model. A burst loss scalar $x$ is introduced that indicated the correlation between average packet loss $\pi_B$ and the probability of loss after a successful transmission $r$. The chance of success after a failed transmission, $r$, is tuned to maintain the average packet loss. Both $p$ and $r$ are obtained using
\begin{align*}
    p &= x\pi_B,\\
    r &= 1-x(1-\pi_B).
\end{align*}
For the user study $x=0.25$ was used.
\begin{figure}[t]
    \centering
    \usetikzlibrary{automata, positioning, arrows}
    \begin{tikzpicture}[scale=1, every node/.style={scale=1}, yscale=1]
    
    \node[state] (q1) at (0,0){$\pi_G$};
    \node[state, right of=q1] (q2) at (1,0){$\pi_B$};
    \draw [->](q1) edge[above, bend left] node{$p=x\pi_B$} (q2);
    \draw [<-](q1) edge[below, bend right] node{$r=1-x(1-\pi_B)$} (q2);
    \draw (q1) edge[loop left] node{$1-p$} (q1);
    \draw (q2) edge[loop right] node{$1-r$} (q2);
    \end{tikzpicture}
    \caption{Diagram of the Gilbert Elliot model and inclusion of scalar $x$ that allows one to change the distribution between burst and uniform behavior without affecting the average packet loss. $\pi_G$ and $\pi_B$ are the average probability of a successful and failed packet transmission respectively. $p$ and $r$ are the chance of switching states. }
    \label{fig:my_label}
\end{figure}
%
\subsection{Experiment design}\label{sec:experiment_design}
%
\begin{comment}
\begin{enumerate}
    \item The environment in which users perform their test cannot be arbitrary
    \item There are several factors that can potentially affect the test results
        \vspace{0.1cm} \hrule \vspace{0.1cm}
    \item \textbf{One:} Tactile Internet is most relevant when there is force feedback. Whenever no interaction with a virtual physics object is occurring, the user cannot observe problems that would be clearly noticeable otherwise.
    \item to partially address this the user should be incentivized to continuously interact with physics objects during the test.
        \vspace{0.1cm} \hrule \vspace{0.1cm}
    \item \textbf{Two:} If left alone different users will do different things. This can sometimes lead to wildly different experiences. The resulting data and user grades experience increased variance because of this.
    \item Users should be incentivized to perform similar motions so that the experience for different users is similar.
    \item note for discussion: that also makes the result more specific, which is worth pointing out. The decrease in variance is desirable during a pandemic, requiring less people for a clear trend, but a follow-up more generalized study is highly desirable.
        \vspace{0.1cm} \hrule \vspace{0.1cm}    
    \item An important point is how the Chai3D physics engine works and what type of data Novint Falcon supplies.
    \item The Novint Falcon provides positional data. This is not how our real bodies work as we apply force. 
    \item the position is placed in the virtual environment, and based on virtual springs, a force reaction is calculated. 
    \item A more rigid surface will be represented by a stiffer virtual spring.
    \item it should be noted that this spring mechanic when using stiff springs in combination with delay, can lead to extreme force feedback values.
    \item As of now it is not clear whether different kinds of physics calculations will exist in the future that suffer this problem less significantly.
    \item if such a system will be adopted in the future, it is possible that the significance of delay in this experiment is overemphasized.
            \vspace{0.1cm} \hrule \vspace{0.1cm}    
    \item \textbf{Subjects}: need to talk about demographic, whatever it is
    \item corona virus limits subjects. A larger sample size is needed for some conclusions, but this work still has value to get the ball going.
\end{enumerate}
    % \item Instead of playing around with block the user has to do a challenge
    % \item The challenge should not be hard but requires focus
    % \item the point is that with a heightened focus and more subtle movement, smaller details can be noticed. 
    % \item walk through one sample of a data point
% \end{itemize}
\end{comment}
%
The experimental setup should provide a platform to facilitate subjective analysis. The setup is designed so that human operators can experience TI sessions and grade them based on user experience. We use this setup to demonstrate the efficacy of ETVO quantitatively. There are a few requirements for an experiment that benefit the statistical relevance of the test results. The first requirement is that the session should incentivize participants to perform the same precise task. The second requirement is that in order to sense minute differences, the participants need to concentrate. This type of concentration would be realistic in mission critical scenarios like telesurgery. However, it is reasonable to expect that the participants of our experiments are not as highly skilled as the surgeon. Hence, it is important that the experiment be designed such that the participants are able to concentrate well without placing high demands on their skill levels. To this end we designed a task that requires the participant to push a cylindrical slider, labeled B in Figure~\ref{fig:ingame}, left and right. A green target is projected onto the plane. During the test, the target moves left and right with smooth transitions. The participant is tasked with pushing the slider around so that it tracks the target as closely as possible. This task is one that most human testers can perform decently well without a lot of explanation or extensive practice. Also, the requirement of tracking the target as closely as possible, means that there is a high skill ceiling. As a consequence, any operator regardless of skill, will be challenged and therefore will concentrate. Finally, the task enforces the operator to continuously interact with the slider, which means that there is haptic feedback for a significant duration of the experiment. Haptic and visual feedback have different requirements, and considering haptic feedback is the main focus, having a lot of physical interaction is desirable. This is important because there is only a limited amount of time participants can continuously do the test, due to the strain on the arm and shoulder, especially for older people. Because every session takes only 20 seconds, multiple sessions with different network settings can be tested. A snapshot from the Chai3D engine is shown in Figure~\ref{fig:ingame}.
\begin{figure}
    \centering
    \includegraphics[trim=0 0 0 170, clip, width=0.5\textwidth]{fig/chai3d_ingame.png}
    \caption{A screenshot of "target tracking" game developed for the subjective performance evaluation of ETVO. A is the target, that needs to be tracked by the slider indicated with B. C is a plane that serves as a rigid floor. The wooden texture is only visual. D is the cursor that represents the position of the Novint Falcon in the virtual environment. A downward line and a shadow are cast on the plane to help the participant understand the 3D location better.}
    \label{fig:ingame}
\end{figure}
% The experiment involves a very specific task and therefore it is important to recognize that this limits the extent to which these results generalize a more broad range of tasks. 
% First of all, the task of pushing a cylindrical slider around is highly specific. Therefore it could be that findings based on this task don't generalize well to a wider range of tasks. Secondly, there is a problem related to how the digital twin is set up. The Haptic device, in this case the Novint Falcon, measures positional data and not the exerted force of the participant. In the physics engine, the location of the ball is replicated. If the ball overlaps with another physics object an imaginary spring is extended based on how deep the sphere penetrates the other physics object. Based on the extension of the spring and the stiffness of the physics object a force is calculated that is fed back to the Novint Falcon. A rigid surface will be represented by a very stiff spring, so the moment the sphere only slightly penetrates the object, a significant response can be generated. This type of calculation is very common, but it should be noted that a spring-based system with rigid surfaces in particular, is highly sensitive to delay, because the stiff spring can be extended before the force feedback is applied. This results in a ``bounce" effect, where the sphere cannot comfortably rest on a rigid surface. Stated differently, the combination of a spring and a delay can make it so that the feedback force is significantly larger than the input force applied by the participant.
%
\subsection{Experiment Procedure}
For the experiment, the participant is informed that the goal of the test is to find out whether they can notice certain disturbances, and whether those disturbances negatively affect their performance. Then the participant gets as much time as they want to familiarize with the application with a perfect network (zero delay and zero loss). On average this takes between 2 and 5 minutes. After the practice round, the participants are given an explanation about the grading process and are told that they should rate the application. After that a series of 20 s tasks is given with each a random network setting. Participants can select a score from 1-10. An indication of how the user grade correlates with user opinion is shown in Table~\ref{tab:user_grade}. A range of 10 values was provided instead of the 5 star system to give the participants more dynamic range to express their opinion.
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}\hline
        % grade & interpretaiton 
        10 & No perceivable impairment \\\hline
        8-9 & slight impairment but no disturbance \\\hline
        6-7 & perceivable impairment, slight disturbance \\\hline
        4-5 & significant impairment, disturbing \\\hline
        1-3 & extremely disturbing \\\hline
    \end{tabular}
    \caption{Correlation between user grade and user opinion.}
    \label{tab:user_grade}
\end{table}
%
\subsection{Participants}
The study contains eleven participants ranging from 20 to 64 years old, with an average age of 31. Out of these five participants had no experience with the device, while six had at least two hours of experience. No participant suffered from known neurological disorders. It should also be noted that most of the data presented in this paper were collected during the COVID-19 pandemic. At all times, the safety regulations issued by the state were maintained, and extra care was taken to disinfect the equipment liberally and often. Because of these concerns, the number of participants is limited and this invites future research with more extensive data sets.

%
% \\ \\
% \textbf{spring physics}
% \begin{itemize}
%     \item force cannot be sensed on the input therefore the is only position
%     \item the position is translated into force by making use of virtual springs
%     \item as a consequence physics are inherently never correct.
%     \item pressing a string with delay means that the reaction comes late: a string can be pressed further than it probably should
%     \item this concept is more true the stiffer the string gets
%     \item the force produced can therefore be much-much higher than put in by the user
%     \item it is very important to understand that this behavior might not be present for any form of TI and can also be a consequence of how physics is implemented. This behavior might not even be what happens in real physics
%     \item however, we might make the assumption that anything that happens here is loosely correlated to other situations. Maybe this is a relatively pessimistic scenario
% \end{itemize}


==> sec/performanceanalysis.tex <==
% \clearpage
%
%
\section{Performance analysis}\label{sec:results}
\begin{figure*}[t]
    \centering
    \includegraphics{fig/paper_header.jpg}
    \caption{Caption}
    \label{fig:examples}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.51\textwidth]{fig/user_study-copy.pdf}
    \caption{The data from all participants are aggregated and shown using a box plot. The horizontal axis shows a range of network settings that where presented to the participant. Column (a) is variable amounts of constant delay. Column (b) is a combination of delay and uniform packet loss. Column (c) is uniform packet loss. Column (d) is bursty packet losses according to the Gilbert Elliot model, where the average packet loss is modulated. Column (e) uses Deadband. The percentage indicates the strength of the Deadband protocol. Column (f) is a combination of 10\% deadband and uniform packet loss. A collection of analytical data is displayed on multiple rows. The first row shows user grades that where provided by participants, and indicates quality of user experience. The second ad third row indicate parameters derived from ETVO, which are average ETO and average EVO respectively. The fourth row indicated RMSE. The last row indicates the average number of packets that where received per second}
    \label{fig:results}
\end{figure}

% \subsection{varying the existing network parameters}
% \begin{itemize}
%     \item first discuss interesting observations that aren't related to evaluation. For example. deadband is more consistent.
%     \item show how packet loss, jitter and delay affect user satisfaction. 
%     \item draw some conclusions over how important delay and unimportant the others are
%     \item [?] see what existing methods make of the data
%     \item illustrate that ETVO agrees, how ETVO views things, what we can learn/conclude etc.
%     \item [?] discuss how ETVO has a better grasp on what is going on than the other methods
% \end{itemize}
\subsection{Fine-grained analysis}
For this work we made alterations to the base DTW algorithm that can be categorized into two groups. The first group of alterations concerns a rewrite of the general structure which transforms the algorithm into a heterogeneous structure. An important aspect is that unlike DTW, ETVO has the ability to select any part of the target sequence to have any delay. The second addition is the addition of penalties. The penalties are responsible for significantly improving the fine-grained analysis. We picked four fragments of time, each corresponding to a different signal. The fragments are picked to illustrate different aspects of decision making between DTW and ETVO, and the effect these penalties have.
%
We start by gauging the sensitivity of each of the schemes to the signal variations. For this experiment, we set the following configuration: 
\textbf{[delay, jitter, $P_\text{prop}$, $P_\text{fixed}$] = [\SI{15}{ms}, \SI{10}{ms}, \SI{0.01}{}, \SI{0.005}]}.
Figure~\ref{fig:examples}(a) corresponds to this experimental setup. It can be observed that when the velocity is high (extremes of the plot), ETVO shows fluctuations in time-offset estimation, but the frequency is significantly reduced in areas with small velocity. This behavior matches with the concept that the effect of jitter is less significant when the velocity in the signal is low.  On the other hand, DTW continuously fluctuates irrespective of context. The scenario for $P_\text{slack}=0$ is also demonstrated (labelled as 'NoSlack'). In this signal, a change in delay is randomly made in the middle of the quiet period (as indicated with 1), while the ETO with $P_\text{slack}$ postpones that decision to a more sensible moment. Note that in the value domain, ETVO and DTW perform similar, despite the significantly higher number of delay adjustments performed by DTW. Moreover, DTW lets the delay fluctuate regardless of what is going on, while ETVO modulates the delay only at high velocities. ETVO reasonably concludes that a higher update rate is desired when more is happening. This example shows how ETVO makes evaluations that are context-aware.  

We now investigate the ETVO performance in the presence of fewer haptic updates. This could be a consequence of either packet losses or employment of compression schemes. To capture the effects of these phenomena, we emulate this scenario through two processes: perceptual deadband \cite{Vittorias2009} and packet losses. This enables us to evaluate the performance when the value-offset is considerable. We choose a deadband of \SI{5}{\%} and bursty loss following the Gilbert-Elliott model with parameters $p=5\%$ and $r=50\%$, as prescribed in \cite{Ellis2014}. For this experiment, we set the following configuration:
\textbf{[delay, jitter, $P_\text{prop}$, $P_\text{fixed}$] = [\SI{00}{ms}, \SI{00}{ms}, \SI{0.005}{}, \SI{0.005}]}.
Figure~\ref{fig:examples}(b) corresponds to this scenario.
It can be clearly seen that the output signal is subject to a noticeable jitter due to the combined effect of packet loss and deadband.
However, there are three specific instances (indicated by markers 2-4) where the combined effect of deadband and bursty losses prominently results in no change in the output signal.
In this case, DTW relentlessly adjusts the time-offset as the deadband and losses are slightly degrading the signal. 
ETVO, however, remains robust to the jitter for the most part and sits at the average delay. But in cases where the effect is prominent, ETO is adjusted as indicated with markers 5-7. 
The value-offset is smoothed with a Gaussian distribution for visual clarity. 
As one expected, in the value domain ETVO is slightly higher than DTW. Although each of the schemes perform their corresponding tasks accurately, the behavior that is most favorable for TI applications is exhibited by ETVO. Especially considering that time variations are considered to be extremely detrimental to the session quality.
%

In this part we show the distinct effects of $P_\text{prop}$ or $P_\text{fixed}$, and the need of considering both. We show the results in Figure~\ref{fig:examples}(c). 
We consider three different settings for algorithm parameters: \\(i) \textbf{[$P_\text{prop}$, $P_\text{fixed}$]} = [0.025,0.05] (corresponds to black curve), \\(ii) \textbf{[$P_\text{prop}$, $P_\text{fixed}$]} = [0.05,0] (corresponds to amber curve), and \\(iii) \textbf{[$P_\text{prop}$, $P_\text{fixed}$]} = [0,0.1] (corresponds to green curve).  Marker 7 indicates an event where the ETO with $P_\text{fixed}=0$ adjusts in multiple small steps. In this case, there is no difference in extra cost associated with using multiple steps, causing the amount of adjustments to increase. Marker 8 indicates an event where the ETO with $P_\text{prop}=0$ causes a large step changes but limited in the number of steps. In this case, there is no extra cost associated with how much the ETO changes, giving rise to giving rise to unreasonably large ETO adjustments. The signal that has both components has a similar performance in the value domain, but a significantly less cluttered ETO. 
%
Figure~\ref{fig:examples}(d) shows the effect that high-frequency noise has on DTW and ETVO. For this purpose, we introduce AWGN with an SNR of \SI{70}{dB}. The experimental configuration is as follows:
\textbf{[delay, jitter, $P_\text{prop}$, $P_\text{fixed}$, $P_\text{slack}$] = [\SI{15}{ms}, \SI{1}{ms}, \SI{0.005}{}, \SI{0.01}{}, \SI{0.005}{}]}.
Both DTW and EVO are plotted with the noise added, while $\text{DTW}_{!N}$, is a version of DTW without the added AWGN. High-frequency noise is a good example of a common way of signal distortion that DTW cannot deal with properly. Note that ETO outperforms the best case DTW i.e. $\text{DTW}_{!N}$, demonstrating its noise resilience. Further, one can also notice the vulnerability of DTW to even a marginal amount of noise causing time-offset to fluctuate vigorously.  
%
\subsection{User study}
ETVO introduces a novel way of evaluating TI sessions, providing a new paradigm for evaluating TI sessions, radically different than the existing QoE and QoS methods. In order to demonstrate ETVO's effectiveness in estimating user satisfaction and its advantages against QoE and QoS a user study was performed. Figure~\ref{fig:results} shows the results of the user study. The data from all participants were aggregated and plotted using a boxplot method. The different types of network settings are separated through different columns. Different extracted statistics are separated by rows. The network settings are described in more detail in Section~\ref{sec:experiment_design}. The ETVO penalties  a constant set is used with \textbf{[$P_\text{prop}$, $P_\text{fixed}$] = [\SI{0.005}{}, \SI{0.005}]}.

First we will analyze the performance of ETVO with respect to QoE based methods. As a representative of this category we use RMSE. This doesn't mean that RMSE is the most sophisticated solution. However it is a good, easy to understand example that shares the same fundamental problem found in other QoE approaches. RMSE performs a sample-to-sample comparison but fails to take into account the time domain. As a consequence, when delay is present, the RMSE output becomes strongly correlated with the time-derivative of the modality. If the time-derivative, which is velocity when tracking position, is high, then a shift in the temporal domain can yield a significant mismatch. In Figure~\ref{fig:results} only column (a) and (b) have an added delay. Here (a) only has delay and (b) has a combination of delay and packet loss. In both these columns one can observe that RMSE has a significant variance, which cannot be found in either EVO or ETO. The variance is mostly because when delay is present RMSE is highly correlated with velocity , which varies from user to user, and even per data point. It should also be noted that for this specific test the velocity was relatively limited. Because the user has to track a target that has a defined speed that is the same for all participants, the velocity as a consequence is quite similar. A more realistic scenario would have significantly higher variance in velocity, which would be reflected in the accuracy of RMSE. This analysis demonstrates that in the event of delay, which will always be present, ETVO manages to find a significantly more precise conclusion than RMSE. An alternative idea to improve RMSE could be to combine RMSE with timestamped delay information. This idea would essentially be a different method to get an ETO estimate. For simple systems this approach would most likely perform very similar to ETVO. However, we expect that in the future more sophisticated TI systems will have to make use of prediction techniques, and various kinds of artificial intelligence, in order to meet the harsh performance requirements. In these cases timestamps would be inadequate leading to the same problem as before. However, ETVO doesn't use predetermined delay information and instead computes it, so ETVO can still fully appreciate the effects of these systems.

Second we will analyze the performance of ETVO with respect to QoS. In this case, the settings of the network are known, because they are used as input parameters. The first observation can be found by comparing the uniform packet loss and bursty packet loss columns, columns (c) and (d) in Figure~\ref{fig:results} respectively. Both the uniform and bursty loss have the same average packet loss, but the bursty loss version performs significantly worse. A reasonable point can be made that it is possible to estimate the amount of bursty loss. However, there are also different ways information can be lost. For example when deploying Deadband, packets are consciously omitted which, when not considering the data, appears as an unpredictable communication pattern. Columns (e) and (f) in Figure~\ref{fig:results} feature Deadband without and with packet loss respectively. One can clearly see that for Deadband without loss, the packet rate is dropped significantly without significant reduction in user grade. However, when combined with some packet loss, the user grade plummets. ETVO can recognize the differences between all of these styles of information loss, and still accurately reflect user grade. However, methods to accurately reflect the user grade using only network parameters is extremely challenging and will only get more challenging as more sophisticated TI systems are developed.



==> tkz/input.tex <==
\newcommand{\vertB}{
(1,0.500),
(2,0.500),
(3,0.500),
(4,0.500),
(5,0.007),
(6,0.005),
(7,0.009),
(8,0.017),
(9,0.020),
(10,0.027),
(11,0.021),
(12,0.075),
(13,0.010),
(14,0.044),
(15,0.001),
(16,0.134),
(17,0.121),
(18,0.228),
(19,0.307),
(20,0.410),
(21,0.440),
(22,0.448),
(23,0.516),
(24,0.535),
(25,0.744),
(26,0.745),
(27,0.704),
(28,0.802),
(29,0.908),
(30,0.944),
(31,1.000),
(32,1.000),
(33,1.000),
(34,1.000),
(35,1.000)
}


==> tkz/output.tex <==
\newcommand{\vertA}{
(1,2.500),
(2,2.500),
(3,2.500),
(4,2.500),
(5,2.500),
(6,2.500),
(7,2.500),
(8,2.014),
(9,2.039),
(10,2.075),
(11,2.022),
(12,2.045),
(13,2.015),
(14,2.014),
(15,2.007),
(16,2.001),
(17,2.034),
(18,2.011),
(19,2.113),
(20,2.225),
(21,2.303),
(22,2.429),
(23,2.507),
(24,2.629),
(25,2.735),
(26,2.805),
(27,2.921),
(28,3.000),
(29,3.000),
(30,3.000),
(31,3.000),
(32,3.000),
(33,3.000),
(34,3.000),
(35,3.000)
}

